Learning to connect in action: Measuring and understanding the emergence of boundary spanners in volatile times

Collective intelligence of diverse groups is key for tackling many of today's grand challenges such as fostering resilience and climate adaptation. Information exchange across such diverse groups is crucial for collective intelligence, especially in volatile environments. To facilitate inter-group information exchange, Informational Boundary Spanners (IBSs) as pivotal information exchange 'hubs' are promising. However, the mechanisms that drive the emergence of IBSs remain poorly understood. To address this gap there is first a need for a method to identify and measure the emergence of IBSs. Second, an Agent-Based Modelling (ABM) framework is not available to systematically study mechanisms for the emergence of IBSs in volatile environments. Third, even though the ability to learn who provides high-quality information is thought to be essential to explain the emergence of IBSs, a rigorous test of this mechanism is missing. The learning mechanism is formalized using an ABM framework, with the model's outputs analyzed using the proposed IBS emergence measurement method. To illustrate both the method and the learning mechanism, we present a case study focused on information sharing in the volatile environment of a disaster. The study shows that learning constitutes a mechanism for the emergence of effective IBSs in (a) low-volatility environments characterised by low uncertainty and (b) in high-volatility environments characterised by rapid change if the number of inter-group connections is sufficient. With the method and model, this paper aims to lay the foundations for exploring mechanisms for the emergence of IBSs that facilitate inter-group information exchange. This article advances collective intelligence by providing the essential elements for measuring and understanding the emergence of IBSs and exploring the effect of learning on their emergence in volatile environments.

==> stuff_spillover_effect.tex <==
In their study, \citet{hazy_impact_2003} found that the required number of nominated boundary spanners increases with higher environmental turbulence. This means that when the environment changes more rapidly and thus generates relevant information with higher frequency, a greater number of boundary spanners is required to successfully find this external information from the environment. \citet{hazy_impact_2003} considered boundary spanners as predefined roles rather than as an emergent phenomenon that may be influenced by environmental turbulence.  Further, their study did not account for the extreme environmental turbulence that can occur during disaster response. In such situations, the amount of information that needs to be managed can be so prominent that actors reach their cognitive load limits, which degrades their ability to find and share information \citep{comes2016cognitive, van2016improving}.

Considering that IBSs tend to process and exchange a high volume of information across different groups, they are likely to become overloaded with information. When the available IBSs are no longer able to provide the information needed, the actors requiring information from them will adapt their information sources to find other actors able to provide information of high quality. This may lead to the emergence of new boundary spanners who %may not have the high level of network centrality of the previous ones, but because of such property, 
are not yet overloaded and can support the exchange of information. Then, a spillover effect is expected such that, with higher environmental turbulence, information boundary-spanning activities are distributed across a higher number of IBSs who "share" the cognitive load of managing inter-group information exchange and processing. %Further, the authors assumed that the amount of connections available between different groups is limited and constant as new connections cannot be established in the short time span occupied by the early phases of a disaster. In such situations, the authors expect that, once the number of emerged IBSs approaches the total number of contacts available among groups through the spillover effect, the number of IBSs reaches a plateau. The following proposition is posited. 

%At the same time, \citep{hazy_impact_2003} did not account for the extreme environmental turbulence that can occur during disaster response. In such situations, the amount of information that needs to be managed can be so prominent that actors reach their cognitive load limits, which degrades their ability to find and share information \citep{comes2016cognitive, van2016improving}. Considering that IBSs tend to process and exchange a high volume of information across different groups, it is expected that they are likely to become overloaded with information. As such, it is expected that the number of IBSs increases when environmental turbulence increases until it plateaus due to information overload. 


%IBSs tend to process and exchange a high volume of information across different groups. As such, it is expected that IBSs are among the most likely actors to become overloaded with information during disasters, thus reducing their ability to effectively exchange information across different groups. When boundary spanners are no longer able to provide the information required, the actors receiving information from them will adapt their information sources to find other actors able to provide information of high quality. This may lead to the emergence of new boundary spanners who may not have the high level of network centrality of the previous ones, but because of such property, are not yet overloaded and can support the exchange of information. It is also expected that the number of boundary spanners is limited by the number of connections that are available among the considered groups. As such, it is expected that the number of boundary spanners increases when environmental turbulence increases until a plateau is reached. %Then, a spillover effect is expected such that, with higher environmental turbulence, boundary-spanning activities are distributed across clusters of boundary spanners who "share" the cognitive load of managing inter-group information exchange and processing.  

%\begin{proposition}[Spillover effect] \label{proposition:et1}
\vspace{3mm}
\noindent 
\textbf{Proposition 3 (Spillover Effect):}
\textit{The emergence of informational boundary spanners increases with environmental turbulence to share the increased cognitive load until it plateaus due to the increased information load and the maximum number of contacts available across groups.}
%\end{proposition}
\vspace{3mm}


Comments about the proposition above: 
You: You need to pick this more apart: 

Nov 20, 2023 6:52 PM • Edit • Delete
You: 1. For the same level of turbulence, when there are more IGCs then the load is shared among more ctors that emerge as IBSs until a plateau is reached (there is no more need for IBSs).

Nov 20, 2023 6:53 PM • Edit • Delete
You: 2. for the same level of IGCs. The higher the load there more the toal load at the boundary tends to be shared among  higher number of actors (the percentage in the histogram is more uniformly distributed) . Need to do a different histogram here :)

Nov 20, 2023 6:54 PM • Edit • Delete
You: 3. for the same level of IGCs and turbulence, the higher the cognitive load limit the more pek IBSs can handle a higher percentage of the total load.

Nov 20, 2023 6:56 PM • Edit • Delete





\section{Discussion}

Figure \ref{fig:spillover-effect} shows that the number of IBSs that emerge increases with the level of environmental turbulence until it reaches a plateau. The figure also shows that the total number of connections is never reached on average. %only for low numbers of inter-group connections available (i.e., in the case of 2). 
This result remains valid also for higher levels of inter-group connections, showing that the number of inter-group connections is not the only limiting factor in the emergence of key IBSs among different groups. Another finding from Figure \ref{fig:spillover-effect} is that the levels of environmental turbulence higher than 10 events per day, the rate with which the growth in emergent IBSs is drastically reduced if not stopped. This shows that for the number of IBSs emerging through the spillover effect tends to reach a plateau depending on the total number of inter-group connections and the considered cognitive load limit. Specifically, the higher the cognitive load limit the higher the highest number of IBSs will be. Further, Figure ... also shows that at higher levels of cognitive load limit, the rate with which the number of IBSs is increasing remains higher, this is particularly the case for numbers of inter-group connections higher or equal to 20. Having a higher capacity to produce more emergent IBSs enables higher performances in general, but specifically, it also enables sustaining a higher level of performance for higher values of environmental turbulence. This can be attributed to the emergence of higher levels of key IBSs through the spillover effect which can manage higher total load at the boundary between the groups. That can, as such, sustain a higher level of performance for the same level of environmental turbulence. This figure only shows the IBSs that manage a peak level of the total information load across the boundary across different groups. Figure ... also shows what percentage of the total load at the information exchange boundary is managed by the 'peak load IBSs'. As it can be noticed, for lower levels of inter-group connections, most of the total load is managed by peak IBSs, however, when the number of inter-group connections increases, the percentage of the total load tends to be more uniform and distributed toward lower percentages of the total load. This shows exactly a spillover effect, meaning that while there are  Peak IBSxs that are very central in that they manage a lot of load individually, a lot of the load can be distributed to the other IBSs that are less central and manage less of the load individually. But, overall these less central IBSs can carry collectively a very high percentage of the total load handled at the boundary between the groups. This pattern is also confirmed when considering the results shown in Figure ..., showing that the average percentage of the total load managed on average by the agents at the boundary between the two groups decreases consistently when the number of inter-group information exchanges. One may imagine that this is due to an increase in agents that handle little to no information. However, even when the trial is cut out (e.g. at a threshold of 3\% this pattern is confirmed. 


%Figure \ref{fig:spillover-effect} shows that the number of IBSs that emerge increases with the level of environmental turbulence until it reaches a plateau. The figure also shows that the total number of connections is never reached on average. %only for low numbers of inter-group connections available (i.e., in the case of 2). This result remains valid also for higher levels of inter-group connections, showing that the number of inter-group connections is not the only limiting factor in the emergence of key IBSs among different groups. Another finding from Figure \ref{fig:spillover-effect} is that the levels of environmental turbulence higher than 10 events per day, the rate with which the growth in emergent IBSs is drastically reduced if not stopped. This shows that for the number of IBSs emerging through the spillover effect tends to reach a plateau depending on the total number of inter-group connections and the considered cognitive load limit. Specifically, the higher the cognitive load limit the higher the highest number of IBSs will be. Further, Figure ... also shows that at higher levels of cognitive load limit, the rate with which the number of IBSs is increasing remains higher, this is particularly the case for numbers of inter-group connections higher or equal to 20. Having a higher capacity to produce more emergent IBSs enables higher performances in general, but specifically, it also enables sustaining a higher level of performance for higher values of environmental turbulence. This can be attributed to the emergence of higher levels of key IBSs through the spillover effect which can manage higher total load at the boundary between the groups. That can, as such, sustain a higher level of performance for the same level of environmental turbulence. This figure only shows the IBSs that manage a peak level of the total information load across the boundary across different groups. Figure ... also shows what percentage of the total load at the information exchange boundary is managed by the 'peak load IBSs'. As it can be noticed, for lower levels of inter-group connections, most of the total load is managed by peak IBSs, however, when the number of inter-group connections increases, the percentage of the total load tends to be more uniform and distributed toward lower percentages of the total load. This shows exactly a spillover effect, meaning that while there are  Peak IBSxs that are very central in that they manage a lot of load individually, a lot of the load can be distributed to the other IBSs that are less central and manage less of the load individually. But, overall these less central IBSs can carry collectively a very high percentage of the total load handled at the boundary between the groups. This pattern is also confirmed when considering the results shown in Figure ..., showing that the average percentage of the total load managed on average by the agents at the boundary between the two groups decreases consistently when the number of inter-group information exchanges. One may imagine that this is due to an increase in agents that handle little to no information. However, even when the trial is cut out (e.g. at a threshold of 3\% this pattern is confirmed. 

%Figure ... shows how the cognitive load limit also reduces the number of IBSs that can emerge before such a number can reach the total number of interconnections among the two groups. %\textit{TODO: discuss figure that shows how for the same number of inter-group connections more IBSs emerge for higher levels of cognitive load limit. This shows that another limiting factor is the cognitive load limit. A third one may be the configuration of the network.}
%Given that, for a number of interconnections that is higher than 2 the number of IBSs that emerged reaches a plateau before reaching the total number of connections, this must be the result of limitation in the cognitive load that the actors can handle rather than the result of network structure. Notably, network structure factors, such as the restricted number of connections among the two groups and their varying degrees of network centrality, are seemingly secondary in explaining this observed behavior.
%This shows that redundancy in the number of connections facilitates the emergence of more IBSs through the spillover effect, thus confirming  Proposition 3. \textit{TODO. Adjust the following argumentation: }

%\textit{TO DO: However, these results do not show that it is the increased cognitive load that causes this. I've run experiments with different levels of cognitive limits. They show that for higher cognitive load limits more IBSs emerge. I expected that higher cognitive load limits would lead to the emergence of fewer IBSs given that one actor can manage more information and thus sharing the cognitive load among multiple actors would be less necessary. However, this is not the case. It seems that higher environmental turbulence provides more chances for a higher number of actors to share external information for the first time, thus leading to a higher number of IBSs. This has nothing to do with Cognitive load. In some cases, the number of IBSs first increases with higher env. turbulence and then it decreases. I suspect this is because of the cognitive load limit. In such cases, the cognitive limit actually reduces the spillover effect for higher levels of env. turbulence. However, this is not a definitive answer yet (needs more work). }

% \subsection{Proposition 4: Peak effectiveness}
% Figure \ref{fig:peak-effectiveness} shows that the effectiveness of IBSs does not present an inverse "U" shape for both shocks and announcements. %Further, a comparison of Figures \ref{fig:peak-effectiveness} and \ref{fig:spillover-effect} shows how, for a level of environmental turbulence between 5 and 10 and number of inter-group contacts higher than 4, the emergence of more IBSs compensates for the increased level of environmental turbulence thus leaving the effectiveness of IBSs roughly constant. However, for higher levels of environmental turbulence (i.e. between 10 and 20) the emergence of new IBSs reaches a plateau and the effectiveness of of IBSs decreases. 
% As such, Proposition 4 is refused for both shocks and announcements. \textit{TODO: I am still wondering if, at 0 announcements or shocks per day, the performance is 0 or 100\%. This would affect the shape of the curves.}

% In the case of shocks, the performance increases and then decreases but at a much slower pace compared to the case of announcements. \textit{TODO: I am still trying to explain this. I thought it was because of learning. But, it is not.}

% \subsection{Proposition 5: Traslation of peak effectiveness}
% Proposition 5 was not confirmed as the results in Figure \ref{fig:peak-effectiveness} shows that the peak does not occur at higher values of environmental turbulence for higher levels of inter-group connections. \textit{TODO: Explain better here with some examples form the graphs.}

% The results in Figure \ref{fig:peak-effectiveness} also show that the effectiveness of IBSs transitions to values above 60 \% when the number of inter-group connections is higher than 10 whereas the effectiveness of IBSs for announcements reaches above 60\% already for 4 inter-group connections. These results show that shocks require higher redundancy than announcements in terms of inter-group connections to guarantee a higher level of peak performance. 
% %In other words, a higher number of inter-group connections is required for shocks compared to announcements. Proposition 5 is modified at this stage based on these findings. 
% An explanation for this finding can be attributed to the different stability in the origin of shocks and announcements. Specifically, in the case of information characterized by a non-stable origin such as shocks, more inter-group connections are required to ensure the same level of effectiveness compared to information with a stable origin such as announcements. This is likely due to the unstable origin that characterizes shocks as they can be introduced at any location of the network, requiring more IBSs to ensure that they reach the professionals. 
% Proposition 5 is modified based on these findings as shown in the following. 

% %\begin{proposition}[Required inter-group connections] \label{}
% \vspace{3mm}
% \noindent
% \textbf{Proposition 5 (Redundancy in interconnections for information of unstable origin):}
% \textit{Fostering the emergence of effective IBSs among groups for information with unstable origin requires higher redundancy in the interconnections among the groups compared to the case in which information has an unstable origin.}
% \vspace{3mm}
% %\end{proposition}

%Further, Figure \ref{fig:peak-effectiveness} also shows that the effectiveness of IBSs for announcements decreases more than for shocks with higher levels of environmental turbulence. A possible explanation resides in the combination of learning behavior and cognitive load. When agents learn the sources from which they can reliably find announcements, they are likely to select the same sources given the stability of information origin. These sources will then be a reference for many actors, leading them to be overloaded with information as information turbulence grows higher. However, in the case of shocks, the sources chosen through learning are likely to be more diversified compared to the case in which announcements are exchanged given the instability in information origin that characterizes shocks. More diversified sources are likely to result in a more distributed cognitive load compared to the case in which announcements are shared, thus enabling the system to sustain higher levels of effectiveness for higher levels of environmental turbulence. Further research is required to investigate if this is actually the case. %Another possible explanation could be the fact that, given that shocks and announcements both take place at the same time, this confuses the actors in 

==> tex_boundary_spanning.tex <==
% boundary spanning mechanisms: boundary spanners and objects
%Different mechanisms for carrying out boundary spanning activities have been individuated in the literature \citep{hawkins2012knowledge}, of which boundary spanners and boundary objects are the most widely studied ones. \textit{Boundary spanners} are the actors that carry out boundary spanning activities. According to previous research, one of the characteristics that boundary spanners should possess to be effective include being recognized as a legitimate participant and having connections in the different groups across which information should be exchanged \citep{tushman1981boundary, levina2005emergence, kim2008formal}. \textit{Boundary objects} are the non-actor entities that support the actors in carrying out boundary spanning activities. According to \citep{star1989institutional}, boundary objects are “\textit{objects that are plastic enough to adapt to local needs and constraints of the several parties employing them, yet robust enough to maintain a common identity across sites}”. Previous studies stress the importance of information technologies such as shared IT applications as Social Media acting as boundary objects \citep{bharosa_netcentric_2011, bharosa2012activity, tim2017digitally}.

%\subsection{Measuring the emergence of informational boundary spanners}\label{sec:em-boundary-spanning}

%\cite{levina2005emergence}  point to boundary spanning as an emergent phenomenon resulting from the decentralized interactions among actors belonging to different groups in non-volatile environments. This pattern was also shown for volatile environments and specifically for disasters by \citep{altay2014challenges} for the 2010 Haiti Earthquake and by \cite{nespeca2020towards} for the case study of Jakarta. The mechanisms through which IBSs emerge are, however, still poorly understood. 
%Modeling and simulation, and especially agent-based modeling and simulation, are powerful tools enabling scientists to investigate mechanisms at the micro level (e.g. adaptation in information sharing preferences) that lead to the emergence of patterns at the macro level (e.g. the emergence of effective informational boundary spanning) \citep{epstein1996growing}. A key first step in studying such mechanisms through modeling and simulation is to find a way to measure quantitatively the emergence of IBSs. \citet{zagorecki_interorganizational_2009} proposes an approach that focuses on monitoring network characteristics such as the average distance between nodes and the average degree in the network. However, such an approach does not enable one to directly measure how many and which agents emerge as IBSs, which is crucial to studying micro-level mechanisms that foster their emergence and to designing effective information management strategies for inter-group information exchange \citep{hazy_impact_2003, altay_information_2013, altay2014challenges}. In sum, a method to directly measure the emergence of IBSs is missing. 


